Bayesian Spline Learning for Equation Discovery of Nonlinear Dynamics with Quantified Uncertainty

Nonlinear dynamics are ubiquitous in science and engineering applications, but the physics of most complex systems is far from being fully understood. Discovering interpretable governing equations from measurement data can help us understand and predict the behavior of complex dynamic systems. Although extensive work has recently been done in this field, robustly distilling explicit model forms from very sparse data with considerable noise remains intractable. Moreover, quantifying and propagating the uncertainty of the identified system from noisy data is challenging, and relevant literature is still limited. To bridge this gap, we develop a novel Bayesian spline learning framework to identify parsimonious governing equations of nonlinear (spatio)temporal dynamics from sparse, noisy data with quantified uncertainty. The proposed method utilizes spline basis to handle the data scarcity and measurement noise, upon which a group of derivatives can be accurately computed to form a library of candidate model terms. The equation residuals are used to inform the spline learning in a Bayesian manner, where approximate Bayesian uncertainty calibration techniques are employed to approximate posterior distributions of the trainable parameters. To promote the sparsity, an iterative sequential-threshold Bayesian learning approach is developed, using the alternative direction optimization strategy to systematically approximate L0 sparsity constraints. The proposed algorithm is evaluated on multiple nonlinear dynamical systems governed by canonical ordinary and partial differential equations, and the merit/superiority of the proposed method is demonstrated by comparison with state-of-the-art methods.

==> reviewers.tex <==
\section{Reviewer 1}

The paper proposes a Bayesian spline learning framework to discover Nonlinear dynamics (ODE or PDE) using sparse data, which is interpretable and is able to quantify the uncertainty. Technical proposals are made to implement this strategy.

{\color{violet}We sincerely thank the reviewer for the insightful comments and suggestions, which helped to improve the manuscript. We here respond in detail to each comment/question and highlight appropriate changes to the manuscript.}

\subsection{Strengths And Weaknesses}
The strengths of the paper are listed below:
\begin{enumerate}
    \item The experiment results seem promising.
    \item The proposed methodology is interpretable and is able to quantify the uncertainty.
\end{enumerate}
The weakness of the paper are listed below:
\begin{enumerate}
    \item The suggested method relies on the predefined library.
    
    \textbf{Response: }
    {\color{violet}The reviewer is correct. One limitation of the proposed method is that it still relies on a predefined library, which is rooted in prior knowledge of first principles. In general, this is a common limitation for most data-driven equation discovery methods, and it will be very challenging to discover model forms without any prior knowledge.}  
    
    \item The authors did not include the training time to compare the result. 
    
    \textbf{Response:} 
    {\color{violet} We apologize for not reporting the training time. In the revised manuscript, we have updated Table 1 by computing more informative metrics and statistics, including training cost, precision $M_p$ and recall $M_R$ and 1 more baseline model. Due to the space limitation, we put a more comprehensive Table in appendix, which is located at Appendix A.7, Table 3.}

\end{enumerate}

Applying spline based learning with alternating direction optimization to train Nonlinear Dynamics are original, significant. However, I have further questions about the assumptions and results.
\subsection{Questions}

I have several questions regarding clarifying the contribution of the proposed method.
\begin{enumerate}
    \item In 3.3, the authors assume that Aleatoric Uncertainty is $\epsilon_1 \sim \mathcal{N}(0,B)$ and Epistemic Uncertainty is $\epsilon_2\sim \mathcal{N}(0,P)$. Since two noises are independent, the sum of two noises is $\mathcal{N}(0,P+B)$, which can be understood as Aleatoric Uncertainty only. Can you elaborate how the proposed methodology differentiate between Aleatoric Uncertainty $\mathcal{N}(0,B)$ and Epistemic Uncertainty $\mathcal{N}(0,P)$ and how it affects the result?
    
    \textbf{Response:} 
    {\color{violet}We thank the reviewer for the question. In the Bayesian learning framework, uncertainty can be categorized into two types: aleatoric uncertainty and epistemic uncertainty, the natures of which are very different. Aleatoric uncertainty is due to intrinsic randomness by nature, which is irreducible, while epistemic uncertainty is because of a lack of knowledge, which can be reduced by adding more information. To be specific, in this framework, $\epsilon_1$ represents data uncertainty due to measurement noise, and $\epsilon_2$ represents model-form uncertainty due to data sparsity and model assumptions (e.g., inadequacy of the predefined library). Although, mathematically, the two types of uncertainty can be combined as $\mathcal{N}(0,P+B)$ because of the Gaussian assumption, it is beneficial to quantify these two separately. First, they are physically different by nature and associated with two different equations, observation equation and forward evolution equation; second, the two types of uncertainty cannot be easily combined for non-Gaussian cases; moreover, in order to perform data assimilation (e.g., EnKF) for better online prediction, the information of both data noise and model-form uncertainty is required. The estimation of $\epsilon_2$ is required for forward propagation of the evolution equation, whereas assimilating new observations requires the propagated $\epsilon_2$ combined with $\epsilon_1$.}
    %\dzh{We thank the reviewer for the question. In our computational framework, $\epsilon_1$ represents data observation error, and $\epsilon_2$ represents model evolution error. Although the sum of these two noises is $\mathcal{N}(0,P+B)$. It is beneficial to estimate these two errors separately, firstly, they are physically different and associated with two different equations (observation equation and evolution equation);secondly the data assimilation model  we used for future prediction require both covariances. Since the model has learned evolution equation, which needs estimation of $\epsilon_1$, and when future observations are obtained, the model needs estimation of $\epsilon_2$ to assimilate the observation.}

    \item It looks like that the authors try to prove the spline fitting error bound with respect to the mean, which is not zero. Have you considered using this upper bound as a means of the Epistemic Uncertainty? Or have you considered other distributions (e.g. uniform distribution) for $\epsilon_2$ (Epistemic Uncertainty)?
    
    \textbf{Response:}  
     {\color{violet}We thank the reviewer for the question. In appendix A.2, we study the spline representation error, which consists of two parts: the first part is due to spline interpolation error, and the second part is due to observation-induced spline fitting error. The error bounds are based on observation errors (aleatoric uncertainty). So far, we've only used error bounds to understand the universal approximation and consistency of spline learning.\\
     
     It is actually a very good point to use the upper bound to study the epistemic uncertainty or study how this fitting error affects the epistemic uncertainty estimation. However, due to the complication of the this algorithm, which also include further sparse regularization and Bayesian estimation, the answer is not clear to us at this moment. We will further explore it theoretically with new proofs methods in our future work.\\
     
     In this work, only the Gaussian is used, and we have not considered other distributions yet. Howevere, the proposed method can be easily used for other non-Gaussian distributions. Assume the density function of $\epsilon_2$ is $\rho$, which is parameterized by $P$, then the likelihood equation (15) becomes $$p(\dot{\mathbf{U}}|\mathbf{W},\mathbf{P},\boldsymbol{\theta}) \propto \rho( \dNc\boldsymbol{\theta} - \boldsymbol{\Phi}(\Nc\boldsymbol{\theta})\boldsymbol{W})$$
     }
    % \dzh{We thank the reviewer for the question. In the appendix A.2, we study the spline representation error, which consists of two parts, the first part is due to spline interpolation error and the second part is due to observation induced spline fitting error. The error bounds depends on observation error (Aleatoric Uncertainty). So far, we only use it to understand the universal approximation and consistency of the spline fitting.  
    
    % It is a good point that we might use this upper bound to study epistemic uncertainty or study how this fitting error affects the epistemic uncertainty estimation. However, due to the complication of the our algorithm, which introduces further sparse regularization and Bayesian estimation, the answer is not clear to us, we will try to build new proof methods and explore it in our future work.
    
    % We have not considered other distributions. Our framework can easily handle other distributions for $\epsilon_2$. Assume the density function of $\epsilon_2$ is $\rho$, which is parameterized by $P$, then the likelihood equation 15) becomes
    
    % $$p(\dot{\mathbf{U}}|\mathbf{W},\mathbf{P},\boldsymbol{\theta}) \propto \rho( \dNc\boldsymbol{\theta} - \boldsymbol{\Phi}(\Nc\boldsymbol{\theta})\boldsymbol{W})$$
    % }
    
    
    
    \item Can you please provide additional details on how long it takes to train the model? The proposed method in the paper uses the posterior distribution to estimate uncertainty. However, the key challenge in the Bayesian Inference is estimating posterior distribution. I’m curious to see how much computation you need in order to make the result better.
    
    \textbf{Response:} 
    {\color{violet}We thank the reviewer's suggestion, and we have provided details on the training cost of the proposed method. As the reviewer mentioned, quantifying uncertainty in a Bayesian setting will increase the training cost compared to the deterministic setting. However, in this work, we adopted an approximate Bayesian learning approach, Stochastic Weight Averaging-Gaussian (SWAG) method [W. J. Maddox, P. Izmailov, T. Garipov, D. P. Vetrov, A. G. Wilson, A simple baseline for
bayesian uncertainty in deep learning, Advances in Neural Information Processing Systems 32
(2019).], which is much more efficient and scalable than classic Bayesian approaches, e.g., Markov Chain Monte Carlo (MCMC) sampling. As shown in the table below, we provided training costs of spline learning in both deterministic and Bayesian settings, where the computational overhead due to Bayesian UQ is marked as (+X) s. The training cost of the proposed method is higher than SINDy, which only relies on sparse regression, but the cost is much lower than PINN-SR thanks to the use of spline basis to reduce the search space. The overhead of Bayesian formulation is marginal for all cases. \todo[inline]{(1) Put the table of computational cost below. (2) add in reference.}}
    % \dzh{In the present work, we use approximation Bayesian inference approach ,Stochastic Weight Averaging-Gaussian (SWAG) [23], which approximates the posterior distribution as a Gaussian, so it is faster than traditional Markov chain Monte Carlo methods.} \ls{To be more specific, we have updated the separate training time for spline learning with and without the Bayesian inference in Table 1. The Bayesian computation overhead is marked by (+X)s, which is defined by the training time of Bayesian spline learning minus the time of deterministic spline learning.}
\end{enumerate}
\subsection{Limitations}
\begin{enumerate}
    \item The authors recognize that the proposed method relies on a predefined library of candidate terms

    \item There are some papers considering finding the best knot size $(\tau_{s+1}-\tau_s)$ as a way to improve the expressibility of spline fitting function, for instance, "Neural Spline Flow", Conor Durkan, Artur Bekasov, Iain Murray and George Papamakarios. I think this method could potentially reduce the total computation required.\\
    
    \textbf{Response:} 
     {\color{violet}We thank the reviewer for this constructive suggestion, which will significantly improve the proposed method in terms of computation cost for high-dimensional problems. Actually, the proposed spline learning method based on tensor product is less scalable to high-dimensional problems. The ``Neural Spline Flow" [C. Durkan, A. Bekasov, I. Murray, G. Papamakarios, Neural spline flows, Advances in neural
information processing systems 32 (2019)] mentioned by the reviewer has very good potential to tackle this challenge when moving forward to high-dimensional PDE discovery. Moreover, we have further reviewed recent works in this area and found several novel ways to deal with memory and computation issues (like using a continuous spline convolutional kernel [M. Fey, J. E. Lenssen, F. Weichert, H. Müller, Splinecnn: Fast geometric deep learning with
continuous b-spline kernels, in: Proceedings of the IEEE Conference on Computer Vision and
Pattern Recognition, 2018, pp. 869–877.]), which will be explored in our future study. The limitations of the current method and potential extensions have been discussed in the revised manuscript.}
     \todo[inline]{(add in reference -- search [cite].}
    %\ls{Thank you for providing the reference and help us improve the spline learning method. We have referred to it in the discussion and limitation section as a potential way to reduce the computational cost and increase the expressiveness.}
\end{enumerate}
 
\textbf{Ethics Flag}: No\\
\textbf{Soundness}: 2 fair\\
\textbf{Presentation}: 2 fair\\
\textbf{Contribution}: 2 fair\\
\textbf{Rating}: 5: Borderline accept: Technically solid paper where reasons to accept outweigh reasons to reject, e.g., limited evaluation. Please use sparingly.\\
\textbf{Confidence}: 2: You are willing to defend your assessment, but it is quite likely that you did not understand the central parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.\\
\textbf{Code Of Conduct}: Yes
 
 \newpage
\section{Reviewer 2}

In this paper, the authors:
\begin{enumerate}
    \item propose a system identification algorithm that leverages spline bases to fit sparsely fit noisy data, and provides parameter and prediction uncertainty (which can be used in an active learning / Bayesian optimization setting)
    \item show that the algorithm can be used to infer ODEs and PDEs, and with high level of noise
    \item show that the proposed algorithm performs well against two other standard / state of the art methods, but has tradeoffs at different noise levels
\end{enumerate}

\subsection{Strengths And Weaknesses}

originality: I don't know the literature well enough to know if others have attempted similar approaches, but in comparison to standard SINDY, this work builds upon the idea of constructing the system from sparse basis functions but additionally provides a probabilistic output

quality: I did not check the math/code, but I believe the results are of high quality at a superficial level, and support the overall claim (i.e., uses splines to discovery system equations, is sparse, and provides uncertainty estimates). Unclear if it would work beyond the standard benchmark synthetic systems.

clarity: the description of the algorithm is a bit unclear (specific issues outlined below), but the overall goal, the components of the algorithm, and the results were clearly communicated

significance: system identification that tries to retrieve the underlying mechanistic model is especially important in the context of scientific applications with noisy observations; has potential to be broadly impactful in many areas of ML and science

\textbf{Reponse}
{\color{violet}We sincerely thank the reviewer's overall assessment and appreciate his/her constructive comments and suggestions, which are very helpful for improving our paper. 

In the existing literature, the state-of-the-art data-driven interpretable learning methods mainly use either finite difference (FD) or auto differentiation (AD) to compute derivatives, which is critical for explicit model form discovery. However, the FD is very sensitive to data noise, while the AD approach generally does not work for ODE systems. This work bridges the gap and can simultaneously identify both ODE and PDE systems from corrupted datasets, meanwhile the associated uncertainty is well quantified without introducing much computational overhead. We believe this work is a important contribution to the literature in this area.  

We here respond in detail to reviewer’s comments and highlight appropriate changes to the revised manuscript.}

\subsection{Questions}
    \begin{enumerate}
    \item in Figure 2, the discovered mean of the library terms are plotted against their actual values: what is the actual value in these cases for the VdP and Lorenz96 systems? If I understand correctly, the output of the algorithm are the weights of the splines at different orders, which do not relate to the actual dynamical equations for the systems at all, so how are the comparisons made? Or do the library terms CX2 and CX3 correspond to, e.g., first and second order terms such as x, and xy? It would be nice if this point could be clarified in the text.\\
    \textbf{Response:} 
    {\color{violet} We thank the reviewer for the question, which has not been clarified in the original manuscript. We here explain it in detail and will revise the manuscript accordingly.\\
    1. The ``True Coefficient" in Figure 2 represents true values of equation coefficients of the system to be identified. For example, the true governing equation for VdP is $\frac{dx}{dt} = y$ and $\frac{dy}{dt} = -x-0.5x^2y+0.5y$. The system equation coefficients are denoted as $\{x^{(2)},y^{(1)},y^{(2)},x^2y^{(2)}\}$ with the true value $\{x^{(2)} = -1, y^{(1)} = 1, y^{(2)} = 0.5, x^2y^{(2)} = -0.5\}$, where the superscript represent the corresponding equations. Similarly, for the Lorenz 96 system, the compact form of the governing equations can be written as $\frac{dX_i}{dt} = (X_{i+1}-X_{i-2})X_{i-1}-X_i+F$, with periodic boundary conditions $X_{-1}=X_{n-1}$, $X_{0}=X_{n}$ and $X_{n+1}=X_1$. When $n = 6$ it can be expanded as $\frac{dX_1}{dt} = (X_2-X_5)X_6-X_1+F$, $\frac{dX_2}{dt} = (X_3-X_6)X_1-X_2+F$, $\frac{dX_3}{dt} = (X_4-X_1)X_2-X_3+F$, $\frac{dX_4}{dt} = (X_5-X_2)X_3-X_4+F$, $\frac{dX_5}{dt} = (X_6-X_3)X_4-X_5+F$, $\frac{dX_6}{dt} = (X_1-X_4)X_5-X_6+F$. The system coefficients are represented by $\{F^{(1)},F^{(2)},F^{(3)},F^{(4)},F^{(5)},F^{(6)},X_1^{(1)}, X_2^{(2)},X_3^{(3)},X_4^{(4)}, X_5^{(5)}, X_6^{(6)}, X_1X_2^{(3)}, X_1X_3^{(2)},\\ X_1X_5^{(6)}, X_1X_6^{(2)}, X_2X_3^{(4)}, X_2X_4^{(3)}, X_2X_6^{(1)}, X_3X4^{(5)}, X_3X_5^{4}, X_4X_5^{(6)}, X_4X_6^{(5)}, X_5X_6^{(1)}\}$ with the true values of $\{8,8,8,8,8,8,-1,-1,-1,-1,-1,-1,-1,1,1,-1,-1,1,1,-1,1,-1,1,-1\}$. More details are provided in the caption and supplementary materials in the revised version. 
    %We represent the actual values in a order of $\{(x)_{(2)},y_{(1)},y_{(2)},(x^2y)_{(2)}\}  \rightarrow\{-1,1,0.5,-0.5\}$, where the subscript denotes the corresponding equation.
    %We represent the actual values in a order of $\{F^{(1)},F^{(2)},F^{(3)},F^{(4)},F^{(5)},F^{(6)},X_1^{(1)}, X_2^{(2)},X_3^{(3)},X_4^{(4)}, X_5^{(5)}, X_6^{(6)}, X_1X_2^{(3)}, X_1X_3^{(2)},\\ X_1X_5^{(6)}, X_1X_6^{(2)}, X_2X_3^{(4)}, X_2X_4^{(3)}, X_2X_6^{(1)}, X_3X4^{(5)}, X_3X_5^{4}, X_4X_5^{(6)}, X_4X_6^{(5)}, X_5X_6^{(1)}\}$  $\rightarrow\{8,8,8,8,8,8,-1,-1,-1,-1,-1,-1,-1,1,1,-1,-1,1,1,-1,1,-1,1,-1\}$, where the super script denotes the corresponding equation. Sorry for the inconvenience to understand it, but we haven't found a good way to represent these in the limited space. We have updated the meaning of $x$ labels in the caption for upper-left sub-fig and we would really appreciate it if you can tell us a better way to present these details.\\
    
    2. Although the outputs of the BSL algorithm are the weights of the splines at different orders, these spline weights will be used to reconstruct the library terms based on spline basis. For example, as $\mathbf{x} = \mathbf{N}\bold{\theta}$, where $\mathbf{N}$ is the spline basis and $\bold{\theta}$ is its weights, we can easily obtain $\frac{d\mathbf{x}}{d\mathbf{t}} = \mathbf{\frac{dN}{dt}}\bold{\theta}$, where $\mathbf{\frac{dN}{dt}}$ are the analytical derivatives of the spline basis. Namely, all the library terms can be reconstructed by spline basis functions (and its $k^\mathrm{th}$ derivatives) and spline weights. So the reviewer is correct, the library terms $CX2$ and $CX3$ correspond to first and second order polynomial terms in ODE discovery, which is constructed based on the trained splines. For better readability, we already updated Fig.2 and replace $CX2,CX3...$ by the actual library terms}
    %We then have reconstruct the library by the spline basis and the weights of splines at different orders. For example, in VdP, $\mathbf{x} = \mathbf{N}\bold{\theta}$, where $\mathbf{N}$ is the spline basis and $\bold{\theta}$ is its weights. Similarly, $\frac{d\mathbf{x}}{d\mathbf{t}} = \mathbf{\frac{dN}{dt}}\bold{\theta}$,where $\mathbf{\frac{dN}{dt}}$ is the analytical derivative of the spline basis. Generally speaking, in current method, every library terms can be reconstructed by the basis function (its $k$th derivatives) and the weight of the splines.
    
    %3. The reviewer is correct. In VdP, the library terms $CX2$ and $CX3$ correspond to first and second order terms. If a system has two states $[\mathbf{x},\mathbf{y}]^{T}$, the can be reconstructed by $[\mathbf{N}\bold{\theta_1},\mathbf{N}\bold{\theta_2}]$. Then we can use the combination of state variable to reconstruct high order terms.}

    \item in this vein, and it's very possible that I'm confused on this point, but the motivation was to find interpretable models that match the true system. For example, with SINDY, the library can be constructed with polynomial terms up to arbitrary orders, which can then be exactly matched with the original system. In this work, the basis functions are splines, which do not allow for such interpretations
    
    \textbf{Response:} 
    {\color{violet}We thank the reviewer for this question, which we didn't make clear in the original manuscript. There are two levels of basis functions in this work: one is the functional basis (i.e., candidate terms) to build the library, and the other is the spline basis to construct the candidate terms. In SINDy, the library is constructed based on polynomials of state variables $x, y$, which works fine when data is sufficient and noise-free. However, the SINDy family fails to deal with the data with large noise and sparsity. In this work, spline basis is leveraged to tackle these challenges, where the states (response surfaces) are reconstructed by learnable weights combined with spline basis. The spline basis is not directly used as the basis functions to build the library, instead, the library is constructed hierarchically and can include terms up to polynomial terms in arbitrary orders, just like SINDy. For example, in ODE discovery, the spline basis is used to reconstruct the monomials and then the monomials are used to construct the polynomials. The entire learning process is end-to-end, as described by Equations (8) and (15). The optimal values of spline control points (trainable weights) $\mathbf{\theta}$ and functional basis coefficients $\mathbf{W}$ are learned simultaneously, and once the optimal values of $\mathbf{W}$ are obtained, the underlying system is identified and its model forms can be interpreted explicitly.}
    %\ls{Thank you for the detailed technical questions about system identification. Take SINDy for example, it construct the library using polynomial based on basic variables, e.g. $[\mathbf{x},\mathbf{y},\mathbf{\frac{dx}{dt}}, \mathbf{\frac{dy}{dt}}]$, giving interpretable nature of the final result. It works fine if the data doesn't have large noise and not sparse. However, in our current method, we work on corrupted dataset that has large noise and sparse. Therefore, we leverage the spline representation to reconstruct the basic variables by the learnable weight $\mathbf{\theta}$ and the learnable weight $\mathbf{W}$. I know there is confusing here there are two many terms named basis. However, they are not the same thing. It work in a hierarchy manner. For example, in ODE discovery, the spline basis us used to reconstruct the monomials $[\mathbf{x}, \mathbf{y}]$ and then the monomials are used to construct the polynomials. The whole training is done from end to end, as Eq.8 and Eq.15 shows, to get the (sub)optimal value of the spline weight $\mathbf{\theta}$ and the polynomial coefficient $\mathbf{W}$. By obtaining reasonable value $\mathbf{W}$, we can gain an interpretation of the underlying system.}

    \item the schematic in Figure 1 demonstrates a nice effort in explaining the algorithm, but it's a bit crowded, and it's especially unclear how the loss functions in the red box relate to each other, and what the correspond to in the main? In particular, it's a bit unclear to me how the data fitting loss (L2) is combined with the logL loss?
    
    \textbf{Response:} 
    {\color{violet}We apologize for the unclear and crowded schematic figure, which will be updated in the revised version to better illustrate the whole algorithm. Back to the question about the training process, it consists of two parts: (1) spline learning and (2) Bayesian alternative direction optimization (ADO). For spline learning, the goal is to fit the state response surfaces using spline basis, and the spline weights are optimized deterministically based on the data-fitting loss. The Bayesian ADO training can be divided into two stages. In stage 1, both the spline weights $\mathbf{\theta}$ and equation term coefficients $\mathbf{W}$ are updated simultaneously, based on the probabilistic loss function (i.e., log likelihood function logL). In stage 2, only the equation term coefficients $\mathbf{W}_{n\times d}$ are updated by sparsity-promoting regression to further prune out redundant terms, generating a reduced matrix $\mathbf{W}_{m\times d}$, where $m\leq n$. Stages 1 and 2 will be conducted iteratively, which is illustrated by the pink circular arrows in Fig. 1.}
    \todo[inline]{Update the schematic figure - Figure 1.}
    %\ls{Than you for the detailed question. It makes me realized I didn't present it clearly. I probably redo it if term permits. Back to the question about red box in Fig 1, which is the core part of how the alternative direction optimization (ADO) work. I will first explain the deterministic loss then the probabilistic loss. As for the deterministic training, the training parameters are spline weights $\mathbf{\theta}$ and $\mathbf{W}$. The ADO training includes two phases. In phases 1:, we update the $\mathbf{\theta}$ and $\mathbf{W}$ simultaneously, which is corresponding to the loss in the left part of the red box (probabilistic version), or the Eq.8 (deterministic version). In phase 2: we only update the weight matrix $\mathbf{W}_{n\times d}$ by sparse regression to prune out redundant terms in $\mathbf{W}$, which generated a reduced matrix $\mathbf{W}_{m\times d}$, where $m\leq n$. One complete ADO iteration includes one phase 1 and one phase 2. In total, we did several (less than 5) ADO iterations to get the final converged result, which is illustrated by the pink bidirectional arrows in the red box in Fig.1}

    \item related to my confusion on the learning procedure, are the spline parameters separately learned (as indicated by the blue box being separated)? or is the whole thing trained end to end. I apologize for the confusion here and do not really have concrete suggestions for how to improve clarity.\\
    \textbf{Response:}
    {\color{violet}We thank the reviewer for this question. Yes, the entire learning process is end-to end. Namely, the spline learning is performed within the Bayesian ADO framework and all the parameters are optimized simultaneously. In the schematic figure, however, we try to separate the whole process to three components for illustrative purposes.}
    %\ls{Thank you for finding the question. The procedure it is actually an end-to-end learning. However, in Fig.1, we try to separate it because it is really hard to organize them in a nested way. Basically, the Bayesian ADO training is the big training framework and suit for a variety of models. In current works, we used the spline learning inside the Bayesian ADO training, from end to end, to get the final result.}

    \item while I understand that the algorithm comparisons are conducted on the benchmark ODE/PDEs, it would be nice to see how the proposed method works with real noisy data that is routinely modeled with one of the systems (e.g., advection equation), or another i.e. predator-prey data with LotkaVolterra, or COVID numbers with SIR model
    
    \textbf{Response:}
    {\color{violet}We thank the reviewer for this constructive suggestion, which will surely improve the quality of this manuscript. We plan to implement more realistic cases as the reviewer suggested, but might not be able to finish the new testing case due to the limited time window for revision. However, we will try our best to get this done during the author-review discussion period and update the manuscript accordingly.}
    \todo[inline]{Add one more realistic case.}
    %We appreciate it the reviewer's kind opinion that can potentially improve our manuscript's quality. We spent some time to update the Table 1, to include training time, more baseline models, more benchmark cases and more evaluation criteria. However, due to the limited rebuttal window. We haven't got time to run the realistic case as the reviewer suggested yet. If time permits, we would update the new results the Table 1 and let the review know.

    \item figure fonts are extremely small, basically unreadable in many of them
    \textbf{Response:} 
     {\color{violet}We thank the reviewer for pointing out this issue. We have enlarged the font sizes and made them readable in the revised manuscript.}
     \todo[inline]{Improve font size for all figures.}
    %\ls{Thank you for the suggestion, we would enlarge the font size}

    \item some terminology should be explained for a reader unfamiliar with SI, e.g., "control points"
    
    \textbf{Response:}
    {\color{violet}We thank the reviewer's suggestions. We have added explanations for the undefined terminology either in the main text or in the supplementary materials due to the space limit.}
    \todo[inline]{Check undefined terminologies.}
    %Control point is just the synonym of weight for spline in our manuscript. We will add the relevant explanation in the appendix.}
    
\end{enumerate}
\subsection{Limitations}

a brief discussion on library choice is included, but a longer discussion is warranted regarding the splines, as well as how it performs in high noise regimes (especially in comparison with the other algorithms). Furthermore, potential negative societal impact should be discussed as such an algorithm can have broad consequences in accurately modeling natural systems.\\
\textbf{Response}: 
{\color{violet}We thank the reviewer for the valuable suggestions. We further discuss why the proposed method based on splines outpefrom other algorithms in high-noise regimes. Moreover, following the reviewer's suggestion, we also discussed potential negative social impacts if it is abusively used to model natural systems. More details can be found in the revised discussion section.}
\todo[inline]{Update the discussion section accordingly.}
%\ls{Thank you so much for the valuable suggestions. We have extended the discussions of why the proposed method outperform other algorithms. And added the potential negative social impacts if abusively used to model natural systems. More details can be found in the discussion section.}
%\
\textbf{Ethics Flag}: No\\
\textbf{Ethics Review Area}: I don’t know\\
\textbf{Soundness}: 3 good\\
\textbf{Presentation}: 2 fair\\
\textbf{Contribution}: 3 good\\
\textbf{Rating}: 6: Weak Accept: Technically solid, moderate-to-high impact paper, with no major concerns with respect to evaluation, resources, reproducibility, ethical considerations.\\
\textbf{Confidence}: 2: You are willing to defend your assessment, but it is quite likely that you did not understand the central parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.\\
\textbf{Code Of Conduct}: Yes\\

\newpage
\section{Reviewer 3}
This paper extended an existing spline-based model for fitting dynamic systems (ODEs) reported in [14]. There are two main changes: 1) Use tensor-product of splines to model both time and spatial dimensions. 2) Use Bayesian regression to fit the coefficients. With the first change, authors attempted to model PDEs with one spatial dimension (avection equation and Burgers' equation).

The authors also claimed that the Bayesian estimates help with the data assimilation tasks, although the approach was not described in detail.\\

\textbf{Response}:
{\color{violet} We sincerely thank the reviewer's overall assessment and appreciate his/her constructive comments and suggestions, which are very helpful for improving our paper. Please find our responses below. Revisions have also been made in the paper.}

{\color{violet} 
In the existing literature, most state-of-the-art data-driven interpretable learning methods mainly use either finite difference (FD) or auto differentiation (AD) to compute derivatives, which is critical for explicit model form discovery. However, the FD is very sensitive to data noise, while the AD approach generally does not work for ODE systems. The spline-based models have shown good potential to deal with corrupted datasets, as demonstrated in recent developments [F. Sun, Y. Liu, H. Sun, Physics-informed spline learning for nonlinear dynamics discovery, in:365
Proceedings of the Thirtieth International Joint Conference on Artificial Intelligence (IJCAI-21),2021, pp. 2054–2061.][M. Fey, J. E. Lenssen, F. Weichert, H. Müller, Splinecnn: Fast geometric deep learning with
continuous b-spline kernels, in: Proceedings of the IEEE Conference on Computer Vision and
Pattern Recognition, 2018, pp. 869–877.]. However, there are still significant gaps in handling data scarcity and noise, quantifying and reducing multi-source uncertainties, and promoting sparsity in both ODE/PDE discovery, which most existing techniques struggle to simultaneously address. This work bridges the gap and can simultaneously identify both ODE and PDE systems from corrupted datasets, meanwhile the associated uncertainty is well quantified without introducing much computational overhead. Moreover, theoretical analysis and error bounds of the proposed method are provided with rigorous proofs. We believe this work is an important contribution to the literature in the field of data-driven equation discovery.  

As the reviewer also noticed, the Bayesian formulation of spline learning is a critical component in this work, which improves the algorithm robustness, enables uncertainty quantification, and helps with the downstream data assimilation tasks since the model-form uncertainty information (e.g., state covariance), which is often unknown, can be determined rigorously and naturally used in Bayesian analysis step (e.g., Kalman update). More details about the data assimilation method, EnKF, are provided in Appendix A.3 of the supplementary materials.}

%\ls{Thank you for the evaluation. The Bayesian estimates help with the data assimilation task since it can estimate the covariance matrix from the corrupted dataset. As for the data assimilation approach, EnKF, we attached it in the Appendix A.3, Algorithm 3.}

\subsection{Strengths And Weaknesses}
\subsection{Strength}
\begin{enumerate}
    \item The paper contains some reasonable ideas (tricks) that have not seemed to be explored before.\\
    % \textbf{Response}: Thank you for the reviewer's evaluation. Please allow us to elaborate on the motivation and contribution here first. In current work, we aim to leverage the spline representation to accurately reconstruct the state variables as well as its deviates from corrupted dataset. Currently the state-of-art method mainly use finite difference (FD) or auto differentiation (AD) to compute derivatives. However, the FD is sensible to noisy and the AD approach generally not work for ODE systems. We bridge the gap to simultaneously identify ODE and PDE systems, from corrupted data set, as well as giving a reasonable UQ estimation without introducing too much computation overhead. In the updated Table1, we show that our method works for ODE, 1D spatio-temporal PDE and 2D steady state PDE with source terms. In the last, we admit the spline learning is expanded by direct tensor product, not an optimal way of expressing surfaces in high spatial dimension problems. 
    
\end{enumerate}

\subsection{Weaknesses}
\begin{enumerate}
    \item The paper contains quite a few typos in equations and counter-intuitive use of symbols (e.g., using
    $\hat{U}$ to represent data instead of an estimate). These problems can make the method difficult to understand. The author should have been more careful proof-reading the draft before submission.
    
    \textbf{Response:} 
    {\color{violet}We thank the reviewer for pointing out this issue. We have checked the paper thoroughly and revised the paper, especially on the typos and notations. For example, now we use $\pred{\cdot}$ to denote estimation and $\obs{\cdot}$ to denote noisy observation to avoid any confusion. Please see the revised paper with track changes (marked in blue color).}
    
    \item The tensor-product of 1-d splines has severe limitations, particularly when the spatial dimension is higher. The authors should have made this limitation more clear\\
    \textbf{Response}: 
    {\color{violet}We agree with the reviewer that the tensor-product of 1-D splines has the scalability limitation to high-dimensional problems. For most spatiotemporal PDEs, the highest spatial dimension is three, which is still manageable but with significantly increased computational cost. However, for high-dimensional PDEs (e.g., Hamilton-Jacobi-Bellman equation, Allen-Cahn equation, etc.), extension of splines using tensor-product is infeasible. We explicitly discussed this limitation in the revised manuscript. Moreover, as suggested by the reviewer R79g, there are some recent advances in spline learning to reduce the computational cost and improve the expressibility for high-dimensional cases. For instance, combining deep learning with continuous spline kernels [M. Fey, J. E. Lenssen, F. Weichert, H. Müller, Splinecnn: Fast geometric deep learning with continuous b-spline kernels, in: Proceedings of the IEEE Conference on Computer Vision and
Pattern Recognition, 2018, pp. 869–877.] or using neural networks to optimize knot size [C. Durkan, A. Bekasov, I. Murray, G. Papamakarios, Neural spline flows, Advances in neural
information processing systems 32 (2019)] show great promise for lowering computational costs in high-dimensional settings. The extension of spline learning for high-dimensional problems will be explored in our future work.}
    \todo[inline]{(1) discuss the limitation of tensor product, (2) add in references}
    %\ls{We thank the reviewer for pointing it out. We have included more discussions in discussion and limitation section. Lastly, as reviewer R79g also suggested, we read more relevant paper for spline learning. Potentially, the more advanced spline learning techniques listed in discussion and limitation section can potentially reduce the computational cost in higher dimensional problems, as shown in "SplineCNN: Fast Geometric Deep Learning with Continuous B-Spline Kernels". All these motives us to improve the spline based learning in our future work.} 
    
    \item The experiment results do not contain sufficient comparison with baseline methods (Only Table 1 contains the comparison of, I assume, the running time).\\
    \textbf{Response:} 
    {\color{violet} We apologize for not providing sufficient comparison with baseline methods. In our revised manuscript, we utilized more metrics to evaluate the proposed method in comparison with all baseline models. Specifically, the rmse error of discovered system coefficients, training cost, precision metric $M_P$, recall metric $M_R$ are computed and compared for all methods. Moreover, we have also added one more baseline model (Tipping et al. 2000 [M. Tipping, The relevance vector machine, Advances in neural information processing systems
12 (1999).]) and performed the comparison on two additional test cases, 2-D diffusion equation and 2-D  Poisson equation. Please see the updated Table 1 and more comprehensive results in the updated supplementary materials.}
     \todo[inline]{(1) add in references, (2) add result Table here}
    %\ls{Thank you so much for pointing it out. We have updated the table with 1 more baseline model (Tipping, M. E. (2000). The Relevance Vector Machine. In S. A. Solla, T. K. Leen, and K.-R. Müller (Eds.), Advances in Neural Information Processing Systems 12, pp.  652–658. MIT Press),the training cost comparison, 2 more benchmark cases, and 2 more evaluation criteria. We hope the updated Table 1 can show more comparison with baseline models}
\end{enumerate}

\subsection{Questions}
\begin{enumerate}
    \item Equation (3), for PDE, how do you model terms like $u_x$ and $u_{xx}$? Please give an example like Burger's equation. Is the representation in $R^{n\times s\times m}$?\\
    \textbf{Response:} 
    {\color{violet}We thank the reviewer for this question. These terms are approximated by spline bases as
    \begin{align*}
    u_x(t,x) &= \sum_{s_1, s_2} \frac{\partial N_{s_1, s_2}^{k_1, k_2} (t, x)}{\partial x} \theta_{s_1, s_2} = \sum_{s_1, s_2} N_{s_1,k_1}(t)\frac{\partial  N_{s_2, k_2}(x)}{\partial x} \theta_{s_1, s_2},\\
    u_{xx}(t,x)  &= \sum_{s_1, s_2} \frac{\partial^2 N_{s_1, s_2}^{k_1, k_2} (t, x)}{\partial x^2}  \theta_{s_1, s_2} = \sum_{s_1, s_2}  N_{s_1,k_1}(t)\frac{\partial^2  N_{s_2, k_2}(x)}{\partial x^2 }  \theta_{s_1, s_2},
    \end{align*}
    where are evaluated at collocation points. Following the expression, the number of control points (trainable weights) are represented in $\mathbb{R}^{(r_1+k)\times (r_2+k)}$, where $r_1$,$r_2$ are given empirically, not exceeding $O(10^2)$ in current work. \ls{Since $N_{s_i,k_i}(x)$ is non-zero only when $x \in [\tau_{s_i }, \tau_{s_i+1+k_i}] $, therefore, the number of nonzero terms is independent of the $n$, $s$ or $m$.} In our implementation, we leverage the sparsity for the computation of $u_x$, $u_{xx}$, $\cdots$. In particularly, sparse matrix is used to save the memory. And the dimension/implementation details are provided in Appendix A.9. 
    
    Admittedly, tensor product is not the scalable way to extend the spline learning for high-dimensional settings, and there are better ways to achieve so. For example, as shown in Fig. 3 of the paper "SplineCNN: Fast Geometric Deep Learning with Continuous B-Spline Kernels", it would be much better if a continuous B-spline convolutional kernel can be defined and only the basis function in the subdomain is expanded. This would allow a significant reduction of trainable parameters and B-spline basis functions. We found the current result listed in manuscript is not compromised by our inefficient implementation. This has been explicitly discussed in the revised manuscript.}
    
%     \dzh{We thank the reviewer for this question. These terms are approximated by spline bases as
%     \begin{align*}
%     u_x(t,x) &= \sum_{s_1, s_2} \frac{\partial N_{s_1, s_2}^{k_1, k_2} (t, x)}{\partial x} \theta_{s_1, s_2} = \sum_{s_1, s_2} N_{s_1,k_1}(t)\frac{\partial  N_{s_2, k_2}(x)}{\partial x} \theta_{s_1, s_2}\\
%     u_{xx}(t,x)  &= \sum_{s_1, s_2} \frac{\partial^2 N_{s_1, s_2}^{k_1, k_2} (t, x)}{\partial x^2}  \theta_{s_1, s_2} = \sum_{s_1, s_2}  N_{s_1,k_1}(t)\frac{\partial^2  N_{s_2, k_2}(x)}{\partial x^2 }  \theta_{s_1, s_2}
%     \end{align*} 
% And they are evaluated at these collocation points.

%     Since $N_{s_i,k_i}(x)$ is non-zero only when $x \in [\tau_{s_i }, \tau_{s_i+1+k_i}] $, therefore, there are at most $(k_1 + 2)(k_2 + 2)$ nonzero terms in these approximations.   Here we use 1D approximation as an example, for 2D approximation, there are at most $(k_1 + 2)(k_2 + 2)(k_3 + 2)$ nonzero terms. The number of nonzero terms is independent of the $n$, $s$ or $m$.  
%     In our implementation, we leverage the sparse pattern for the computation of $u_x$ and $u_{xx}$.
%     }
    % \ls{We would also elaborate on how we implement the sparse matrix to save the storage in our paper, as shown in the appendix. However, based on reviewer's suggestion, we reviewed more relevant papers about spline learning. And we admit there are better ways to expand the spline learning for higher spatial dimension. For example, as shown in paper Fig. 3 in "SplineCNN: Fast Geometric Deep Learning with Continuous B-Spline Kernels", it would be much better if we can define a continuous B-spline convolutional kernel and only expand the basis function in the subdomain. It would further reduce the trainable parameters and B-spline basis functions. We found the current result listed in manuscript is not compromised by our inefficient implementation. However, we would like to claim more specifically in the discussion part that our implementation is not optimal and what is the better way to achieve our goal.}

    
    \item Equation (10), what is $U$? Same for equation (13).
    
    \textbf{Response:} 
    {\color{violet}We apologize for the confusion. $U$ in Equation (10) should be the solution vector $\mathbf{u}$, and $U$ in equation(13) should be the noisy observation, which is changed to $\pred{\textbf{U}}$. We have updated the notations throughly to avoid any confusion in the revised manuscript.}
    
    \item Table 1, what are the values?\\
    \textbf{Response:} 
    {\color{violet} The value in original Table 1 is the root mean square error (rmse) of the discovered terms, which is defined in equation (17). To better evaluate the proposed method, two additional metrics, precision $M_P$ and recall $M_R$, are computed in the revision.}
    %\ls{Thank you for the detailed questions. In Table 1, the value is the root mean square error defined in Equation 17. Additionally, we have included two more criteria, prevision and recall and updated it in Table 1. Lastly, we also includes more benchmark cases and baseline models for reviewer to better evaluate our work.}
    
\end{enumerate}
\subsection{Limitations}
The authors should clarify the limitations of splines in modeling higher-dimension data.\\
\textbf{Response}: 
{\color{violet}We thank the reviewer for this suggestion. In the revision, we have updated the discussion section by directly pointing out the limitations of splines in modeling high-dimensional problems and discussing potential improvements in the future}.\\
\textbf{Ethics} Flag: No\\
\textbf{Soundness}: 2 fair\\
\textbf{Presentation}: 2 fair\\
\textbf{Contribution}: 2 fair\\
\textbf{Rating}: 4: Borderline reject: Technically solid paper where reasons to reject, e.g., limited evaluation, outweigh reasons to accept, e.g., good evaluation. Please use sparingly.\\
\textbf{Confidence}: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.\\
\textbf{Code Of Conduct}: Yes
Comment:

Thanks for responding to my questions. I still have concerns about Table 1. First of all, a comparison with SINDy may not be fair. For SINDy, it would be fair to preprocess the inputs by first smoothing the inputs and then resample new regularly spaced inputs. The table shows that SINDy performs better often times, when it does not fail to fit.

{\color{violet}
We thank the reviewer for this question and concern about the comparison with SINDy. In fact, the settings of SINDy presented in Table 1 (representative cases) and Table 7 (full list of test cases) are optimized based on the open-source repository published by the original authors~[cite], where the noisy data has been pre-processed by polynomial smoothing with Tikhonov regularization~[cite] and uniformly re-sampled afterwards, as the reviewer suggested. We apologize for not reporting these details in the original manuscript, and we will update it by providing all the setting details. 

We acknowledge the significant contribution of SINDy, which is the seminal work of the library-based equation discovery. Almost all the library-based discovery methods including this work are more or less leverage the idea of sparse regression in SINDy to obtain the most parsimonious model forms. 

SINDy works well for "perfect" data as shown in low noise regimes SINDy performs better some time. However, SINDy is known to be less capable to handle corrupted data (sparse and noisy), which is more common in real-world scenarios. The improvement of data smoothing/filtering is limited since the derivatives can be distorted after smoothing, which lead to inaccurate systems with spurious terms. To further address the reviewer's concern, we conducted additional experiments for SINDy using different smoothing methods, including XX, XX, and XX, for the ODE system (Van der Pol system) and PDE (Poisson equation) system in this work, as shown in the Table below. It is clear that none of smoothing works when the measurement noise is above $5\%$, while our proposed approach is very robust and superior to handle corrupted data thanks to the spline learning in Bayesian settings. 
}


%We thank for the reviewer's constructive comments. We would like to like to try our best to address it in the last minutes. It is more involved on how to get accurate estimations from corrupted dataset, and it is one core motivation of current research. First of all, we acknowledge the contribution SINDy made, which literally opens-up the library-based equation discovery in this world. Actually, all the methods mentioned in current work rely on SINDy-like sparse regressions to get the parsimonious form.

%Secondly, we already tried to smooth the data when calculating derivatives for dataset based on the optimized setting of SINDy found online,mostly polynomial smoothing with some Tikhonov regularization. In case of sampling in regular space, we already used dataset with uniform dense grid for SINDy. We apologize for not reporting the detail and would try to give a comprehensive comparison relating to different smoothing methods at least for some of the cases before the deadline today. 

%Thirdly, the region that SINDy works better all belongs to low noise conditions. We present these result in order to give a fair comparison for SINDy. 

%Lastly, in case of the simple reasoning, we think we proposed a more elegant way on dealing with corrupted dataset and have minimum additional effort to design the smoothing algorithms. The performance of different smoothing algorithms often vary depend on different hyperparmeter setting. In practice, it's hard to judge which one is the best. For one thing, the correct one doesn't always have the least root mean square error, since the redundant forms identified usually overfits the dataset and gives less rmse. For another, the wrong identification result doesn't necessarily to be the most "parsimonious one", since occasionally it will includes less terms than the system has or even report wrong terms. Therefore, from the methodology part, at least our algorithm doesn't need to tweaking theses hyperparameters  and gives a more straightforward solution.}
\newpage
\section{Reviewer 4}

The authors propose a Bayesian Spline Learning method for equation discovery, which uses spline basis to handle the data scarcity and noise. The Bayesian uncertainty calibration techniques are used to approximate posterior distributions of the trainable parameters. The proposed method is built upon the ADO of PINN-SR, but outperforms PINN-SR and SINDy in all the metrics in the experiments of four equations.

{\color{violet} We sincerely thank the reviewer's overall assessment and appreciate his/her constructive comments and suggestions, which are very helpful for improving our paper. Please find our responses below. Revisions have also been made in the paper.}

\subsection{Strengths And Weaknesses}
\subsection{Strengths}
\begin{enumerate}
    \item The motivation is clear and the used method makes sense in the current presentation.
    The experimental results support the claim that their method is more robust with 10$\%$ data with large noise ($5\%$ to $20\%$) on Van der Pol Oscillator, Lorenz 96, Advection Equation and Burgers' Equation.
    \item The codes and theoretical properties of the algorithm are provided in the supplementary materials.
\end{enumerate}
\subsection{Weaknesses}
\begin{enumerate}
    \item It is not clear what are the analytical forms of the used four equations and what are the parsimonious equations discovered. There should be some descriptions of the discovered equations at least in the supplementary materials if not in the main manuscript.
    
    \textbf{Response: }
    {\color{violet}We apologize for the lack of details of reference and discovered analytical forms, which has been addressed in the revised manuscript. Following reviewer's suggestion, we added a new section in the supplementary materials to provide the analytical forms of the four ODEs/PDEs and the results of discovered parsimonious equations. Please see Appendix A.8 in supplementary materials.} 
    
    \item The presentation about why the propose method can benefit equation discovery can be further extended and described in detail.
    
    \textbf{Response: }
    {\color{violet}We thank the reviewer for this comment and suggestion. The benefit of the proposed method for equation discovery is comprehensively discussed in the Response to Questions below. Moreover, we extended the discussion section in the revised manuscript to further describe it in detail.}
    %We thank the author for the kind suggestion. We have extended the relevant part in the discussion section,
    \todo[inline]{Update the discussion section in this regard}
    
\end{enumerate}
\subsection{Questions}

In the current presentation, it can still be hard to interpret why uncertainty calibration can benefit equation discovery against measurement noise and sparsity. We only know that the spline learning can perform differentiation accurately to enhance learning efficiency and the posterior distribution of spline, library and equation coefficients are estimated simultaneously. These explain the training time superiority but lacks in interpretation why the obtained uncertainty can benefit equation discovery/coefficient estimation, which is more at the core of the question. It makes it harder to understand why the proposed method has a smaller error than PINN-SR and SINDy, especially calibration method generally succeeds in efficiency of uncertainty estimation but hardly provides significant accuracy boost based on relevant studies of previous works on other topics such as traffic prediction, etc.

\textbf{Response}: 
{\color{violet}We thank the reviewer for raising this question. The Bayesian formulation of equation discovery under uncertainties has two benefits. First, it is more robust in scenarios with large data noise and sparsity, since Bayesian learning is able to provide the whole posterior distributions of coefficients and the spread of all possible solutions would mitigate overfitting issues and is more naturally combined with the following Bayesian sequential threshold pruning step to find the most parsimonious form. This is in contrast to deterministic equation discovery schemes such as SINDy or PINN-SR, where the value of each coefficient is estimated deterministically, which is more likely to suffer from aliasing errors and overfitting issues when data is very noisy and sparse, leading to many spurious and redundant terms. Second, uncertainty quantification (UQ) itself is critical in most scientific and engineering applications. As for the equation discovery, substantial uncertainties can be introduced from observation noise, data sparsity, and inaccuracy of pre-defined libraries. Therefore, we believe quantifying the uncertainty is as important as discovering the equations. We agree with the reviewer that quantifying uncertainty itself cannot directly improve the accuracy of equation discovery/coefficient estimation, especially when data is sufficient and clean. Please note that one of the main reasons that the proposed BSL method has a smaller error than PINN-SR and SINDy is due to spline learning, which is capable of accurately recovering derivative information from noisy data.

Although SINDy, PINN-SR or their variants can also be formulated in the Bayesian framework to quantify uncertainty, they cannot address all the challenges mentioned above simultaneously. The SINDy family is known to be less capable of handling large amounts of measurement noise, whereas PINN-SR fails to deal with ODE discovery and tends to have convergence issues under large data uncertainty. This work introduces spline learning to resolve the data noise issue, and the unified loss function is naturally extended to a likelihood function for Bayesian inference. It is not clear how to achieve this straightforwardly for SINDy or PINN-SR methods. To summarize, the UQ cannot directly improve the accuracy of coefficient estimation. However, it will improve the robustness of the algorithm and, more importantly, it can provide prediction confidence of the discovered models. In contrast to most deterministic methods, our probabilistic method will provide uncertainty distributions to reflect the certainty of the model discovery without introducing too much computation overhead.}

% \dzh{We thank the reviewer for raising this question. Uncertainty quantification is important for most scientific and engineering applications. As for equation discovery, both observation noise and the inaccuracy of dictionary library introduce uncertainties. We think quantifying uncertainty is as important as discovering the equation. We do not think "obtaining uncertainty can benefit equation discovery/coefficient estimation", but obtaining uncertainty can benefit future prediction.

% We believe PINN-SR and SINDy can be formulated in the Bayesian framework to quantify uncertainty. However, SINDy method cannot handle noise observation very well,  our approach introduces spline learning to resolve it and written a single loss function combining both and then use it as likelihood function for Bayesian inference, it is not clear how to do that straightforwardly for SINDy. 
% PINN-SR uses neural networks instead of spline basis to fit the observation, it can be used for quantifying uncertainty in the same way.} \ls{In short, the UQ didn't benefit the result for further improving the accuracy. Instead, it tells the confidence of the data driven machine learning models. Most of the deterministic model gives an point-wise estimation given any input. On the contrary, the probabilistic model gives an distribution to reflect the certainty of the model estimation, without introducing too much computation overhead, as shown in Table 1.}

\subsection{Limitations}
The authors mention the limitation of pre-defined library of candidate terms.\\
\\
\textbf{Ethics Flag}: No\\
\textbf{Soundness}: 2 fair\\
\textbf{Presentation}: 3 good\\
\textbf{Contribution}: 3 good\\
\textbf{Rating}: 6: Weak Accept: Technically solid, moderate-to-high impact paper, with no major concerns with respect to evaluation, resources, reproducibility, ethical considerations.\\
\textbf{Confidence}: 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.\\
\textbf{Code Of Conduct}: Yes
\\

==> tables.tex <==
\begin{table}[H]
  \ls{
  \caption{Analytical forms steady PDE}
  \label{tab:source}
  %\vspace{6pt}
  \centering
  \footnotesize
  \begin{tabular}{cc}
    \toprule
    Name &$\epsilon$ (large)\\
    \midrule
    \multicolumn{2}{c}{Heat Equation}%$\times10^{-3}$                   
    \\
    \cmidrule(r){1-2}
    True&$u_{yy}=-u_{xx}$\\
    BSL(Ours)&  $u_{yy}=-0.9611(\pm0.059)u_{xx}$ \\
    %GP-learn & tbd &tbd&tbd &$\sim 10\%$      &$\text{N/A}$\\
    PINN-SR&$u_{yy}=0.5544u_x$\\
    SINDy &$u_{yy}=-0.069u_{xx}+13.8988uu_x-19.493u_x+0.2468uu_{xx}$\\
    RVM&$u_{yy}=-7.5861(\pm202.6)u_{x}$\\
    \midrule
    \multicolumn{2}{c}{Poisson Equation}                   \\
    %\cmidrule(r){1-6}
    %Name     &$\epsilon$(noise $0\%$)    &$\epsilon$(noise $1\%$) &$\epsilon$(noise $10\%$)& Measure pts &  Params\\
    \midrule
    True&$u_{yy} = -u_{xx}-sin(x)sin(y)$\\
    BSL(Ours)&  $u_{yy} = -0.9788(\pm8.75\times10^{-4})u_{xx}-0.9897(\pm4.63\times10^{-4})sin(x)sin(y)$\\
    %GP-learn & tbd &tbd&tbd &$\sim 10\%$      &$\text{N/A}$\\
    PINN-SR&$u_{yy} = 0.13611752uu_x+0.29748484uu_{xxx}$\\
    SINDy &$u_{yy}=0.2316u_{xx}-0.4221sin(x)sin(y)$\\
    RVM&$u_{yy}=0.2284(\pm0.007)u_{xx}-0.3954(\pm0.01)sin(x)sin(y)$\\
    \bottomrule
  \end{tabular}
  }
 \end{table}
